Fire360: A Benchmark for Robust Perception and Episodic Memory in Degraded 360-Degree Firefighting Videos

Modern AI systems struggle most in environments where reliability is critical - scenes with smoke, poor visibility, and structural deformation. Each year, tens of thousands of firefighters are injured on duty, often due to breakdowns in situational perception. We introduce Fire360, a benchmark for evaluating perception and reasoning in safety-critical firefighting scenarios. The dataset includes 228 360-degree videos from professional training sessions under diverse conditions (e.g., low light, thermal distortion), annotated with action segments, object locations, and degradation metadata. Fire360 supports five tasks: Visual Question Answering, Temporal Action Captioning, Object Localization, Safety-Critical Reasoning, and Transformed Object Retrieval (TOR). TOR tests whether models can match pristine exemplars to fire-damaged counterparts in unpaired scenes, evaluating transformation-invariant recognition. While human experts achieve 83.5% on TOR, models like GPT-4o lag significantly, exposing failures in reasoning under degradation. By releasing Fire360 and its evaluation suite, we aim to advance models that not only see, but also remember, reason, and act under uncertainty. The dataset is available at: https://uofi.box.com/v/fire360dataset.

==> figures/figures.tex <==
Dataset Overview Figure: A visual showing example frames from  dataset highlighting:

Day/night conditions
Indoor/outdoor environments
Varying levels of smoke/visibility
Example annotations with bounding boxes


Object Transformation Diagram: 
A visual sequence showing:

Pre-fire object appearance
During-fire transformation
Post-fire transformed state
Annotation approach for tracking identity


Annotation Tool Interface: Screenshot of web-based tool showing:

The equirectangular projection interface
Annotation modes (temporal, spatial, environmental)
Export capabilities


Benchmark Task Visualization: Diagram illustrating:

Input/output for each benchmark task
Example of Transformed Object Retrieval challenge
Performance degradation under challenging conditions















Sample frames with annotations showing the different visibility conditions

Visualization of the object transformation process (before/after)

Screenshot of your annotation tool interface
Task diagrams, especially for the Transformed Object Retrieval challenge

Your paper would benefit significantly from the following visualizations:

Dataset Examples - Show actual frames from your 360° videos demonstrating:

Varying lighting conditions (day/night)
Smoke occlusion levels
Object transformations (before/after fire exposure)


Annotation Tool Interface - Include a screenshot of your annotation tool showing:

The UI for labeling 360° equirectangular video
Different annotation modes you describe in Section 5


Transformed Object Retrieval Task - Create a visual diagram showing:

Input: Pre-disaster object image
Output: Located object in post-disaster 360° scene
The transformation challenge (perhaps with difficulty levels)


Architecture Overview - Include a system diagram showing:

Data collection pipeline
Annotation process
Benchmark task evaluation flow


Results Visualization - Replace placeholder Table 2 with:

Actual performance metrics
Comparative charts showing model performance degradation under different conditions

==> sections/datasheet.tex <==
\section*{Appendix A: Datasheet for Fire360}

\textbf{Dataset Title:} Fire360: A Real-World 360° Video Benchmark for Safety-Aware Firefighting AI

\textbf{Motivation:}
This dataset was developed to enable research in safety-critical embodied AI systems, particularly for first responder training, episodic memory reasoning, and panoramic scene understanding. It addresses a gap in existing datasets, which are often synthetic, narrow-FoV, or collected under idealized conditions.

\textbf{Composition:}
Fire360 contains 100 real-world 360° videos of firefighter training drills, recorded across daytime, nighttime, indoor, and smoke-filled environments. Each video is approximately 7 minutes long and recorded in 4K at 60fps using a Ricoh Theta 360 camera.

\textbf{Annotations:}
Each video is annotated with:
\begin{itemize}
    \item Temporal action segments (start, end, action label)
    \item Object-level bounding boxes for firefighting gear, tools, and vehicles
    \item Environmental context tags (e.g., smoke, night, indoor)
    \item Transformation annotations for fire-damaged objects (where applicable)
\end{itemize}
Average annotations per video: 3–4 actions, 5–6 objects.

\textbf{Collection Process:}
The data was recorded at one of the oldest firefighter training facilities in the U.S. No civilians or sensitive personal information is present. All recordings were authorized and approved by the training institute’s leadership and project PIs.

\textbf{Annotation Process:}
Annotations were performed by the dataset authors and reviewed by researchers and instructors at the fire training institute. The annotation tool supports multi-level labeling and allows exporting to CSV and JSON formats. No crowd-sourced labor was used.

\textbf{Uses:}
Fire360 is intended for:
\begin{itemize}
    \item Safety-aware vision-language reasoning
    \item Episodic memory and transformed object retrieval
    \item Virtual reality training content generation
    \item Multi-agent coordination and simulation
\end{itemize}

\textbf{Distribution:}
The dataset and annotation tool will be hosted publicly on a platform such as Hugging Face or Kaggle under a research-only license. Code and documentation will be included. A Croissant metadata file will accompany the release.

\textbf{Ethical Considerations:}
We ensured all footage contains no personally identifiable information. Data was collected in controlled training environments with institutional approval. Potential misuse for surveillance or unrelated safety monitoring is explicitly prohibited in the license terms.

\textbf{Maintenance:}
The dataset will be maintained by the authors, with versioned updates and a contact email for reporting issues.


